Recurrent Inference Machines for Solving Inverse Problems

Much of the recent research on solving iterative inference problems focuses on moving away from hand-chosen inference algorithms and towards learned inference. In the latter, the inference process is unrolled in time and interpreted as a recurrent neural network (RNN) which allows for joint learning of model and inference parameters with back-propagation through time. In this framework, the RNN architecture is directly derived from a hand-chosen inference algorithm, effectively limiting its capabilities. We propose a learning framework, called Recurrent Inference Machines (RIM), in which we turn algorithm construction the other way round: Given data and a task, train an RNN to learn an inference algorithm. Because RNNs are Turing complete [1, 2] they are capable to implement any inference algorithm. The framework allows for an abstraction which removes the need for domain knowledge. We demonstrate in several image restoration experiments that this abstraction is effective, allowing us to achieve state-of-the-art performance on image denoising and super-resolution tasks and superior across-task generalization.

==> related_work.tex <==
The RIM framework can be seen as an auto-encoder framework in which only the decoder is trained, whereas the encoder is given by a known corruption process. In terms of the training procedure this makes RIMs very similar to denoising auto-encoders \citep{Vincent2008}. Though initially with the objective of regularization in mind, denoising auto-encoders have been shown to be effectively used as generative models \citep{Vincent2010}. The difference of RIMs to denoising auto-encoders and also more recently developed auto-encoders such as \citet{kingma2013auto,Rezende2014} is that RIMs enforce coupling between encoder and decoder both, during training and test time. In it's typical form, decoder and encoder of an auto-encoder are only coupled during training time, while there is no information flow during test time  \citep{kingma2013auto,Rezende2014,Vincent2008,Vincent2010}. An exception is the work from \citet{Gregor2016} which is conceptually strongly related to RIMs. There, an RNN model is used to generate static data by drawing on a fixed canvas. An error signal is propagated throughout the generation process.

There have been approaches in the past which aim to formulate a framework in which an inference procedure is learned. One of the best known frameworks is LISTA \citep{Gregor2010} which aims to learn a model that reconstructs sparse codes from data. LISTA models try to fit into the classical framework of doing inference as described in \ref{sec:Intro}, whereas RIMs are completely removed from assumptions about sparsity.
A recent paper by \citet{Andrychowicz2016} aims to train RNNs as optimizers for non-convex optimization problems. Though introduced with a different intention, RIMs can be seen as a generalization of this approach, in which the model - in addition to the gradient information - is aware about the absolute position of a prediction in variable space(see equation \eqref{eq:update_equation}).
